Boron Nitride Nanotube Peapod under Ultrasonic Velocity Impacts: A Fully Atomistic Molecular Dynamics Investigation

In this work, we investigated the mechanical response and fracture dynamics of boron nitride nanotubes (BNNTs)-peapods under ultrasonic velocity impacts (from 1 km/s to 6 km/s) against a solid target. BNNT-peapods are BNNTs containing an encapsulated linear arrangement of C60 molecules. We carried out fully atomistic reactive (ReaxFF) molecular dynamics simulations. We have considered the case of horizontal and vertical shootings. Depending on the velocity values we observed tube bending, tube fracture, and C60 ejection. One interesting result was tube unzipping with the formation of bilayer nanoribbons 'incrusted' with C60 molecules.

==> rascunhos.tex <==
The versatility of carbon atoms originated from their hybridization states $sp$, $sp^2$ and $sp^3$ generates new remarkable nanostructures, whose syntheses have been drawing special attention in the past 4 decades. These new carbon forms have distinct chemical and physical properties and comprise all dimensionalities such as fullerene (0D), carbon nanotubes (1D) \cite{iijima1993single}, graphene (2D), and graphite (3D). Many of those nanostructures can be combined in a solid form to obtain new materials with desirable mechanical \cite{Vinod2014}, electronical, thermal and magnetic properties using chemical(covalent bonds) or physical (van der Waals interactions).
